PRESISTANT: Learning based assistant for data pre-processing

Data pre-processing is one of the most time consuming and relevant steps in a data analysis process (e.g., classification task). A given data pre-processing operator (e.g., transformation) can have positive, negative or zero impact on the final result of the analysis. Expert users have the required knowledge to find the right pre-processing operators. However, when it comes to non-experts, they are overwhelmed by the amount of pre-processing operators and it is challenging for them to find operators that would positively impact their analysis (e.g., increase the predictive accuracy of a classifier). Existing solutions either assume that users have expert knowledge, or they recommend pre-processing operators that are only "syntactically" applicable to a dataset, without taking into account their impact on the final analysis. In this work, we aim at providing assistance to non-expert users by recommending data pre-processing operators that are ranked according to their impact on the final analysis. We developed a tool PRESISTANT, that uses Random Forests to learn the impact of pre-processing operators on the performance (e.g., predictive accuracy) of 5 different classification algorithms, such as J48, Naive Bayes, PART, Logistic Regression, and Nearest Neighbor. Extensive evaluations on the recommendations provided by our tool, show that PRESISTANT can effectively help non-experts in order to achieve improved results in their analytical tasks.

==> other.tex <==


\begin{algorithm}
%\textbf{Input:} $models[..];$ \Comment{meta-model for each algorithm} \\
%$transformations[..];$ \Comment{set of transformations to be applied} \\
%$ds$ \Comment{new dataset chosen by the user} \\
%$datasets[..];$ \Comment{available datasets of classification type} \\
%$classificationAlgs[..];$ \Comment{available classification algorithms} \\
%\textbf{Output:} $transformations[..];$ \Comment{trans. ordered according to predicted impact}
\caption{Evaluation}
\label{alg:recommending_phase}
\begin{algorithmic}[1]
\Function{Evaluate top-L}{$datasets[]$,$transformations[]$,$classificationAlgs[]$}
    \For {each $l$ in $L$}
        \For {each dataset $ds$}
        \State $ordered.transformations=$ \textproc{OrderByProbability()};
            \If{$real.positives$ in $ds$ $>=$ $L$}
            \State $pos.predictions=$ \textproc{GetPosPredictedTransformations()};
                \If{$pos.predictions >=1$}
                    \If{\#$pos.predictions <L$}
                        \State $new.L =$ \#$pos.predictions$
                    \Else{}
                        \State $new.L = L$
                    \EndIf
                    \State $TP=$ \textproc{GetTP(new.L)}
                    \State $FP=$ \textproc{GetFP(new.L)}
                    \State $posPrec=TP/new.L$ 
                \EndIf
            \Else{}
                \State $continue;$
            \EndIf
        \EndFor
    \EndFor
\EndFunction
\end{algorithmic}
\end{algorithm} 



Precision and recall are the most popular metrics based on this~\cite{Lü20121}.  For a target dataset i, precision and recall of recommendation, $P_i(L)$ and $R_i(L)$, are defined as 
\begin{equation*}
    P_i(L)=\frac{d_i(L)}{L}, R_i(L)=\frac{d_i(L)}{D_i}
\end{equation*}
where $d_i(L)$ indicates the number of relevant transformations (objects collected by $i$ that are present in the probe set) in the top-$L$ places of the recommendation list, and $D_i$ is the total number of $i$'s relevant?? transformations. Averaging the individual precision and recall over all datasets with at  least  one  relevant transformation,  we  obtain  the  mean  precision  and  recall, $P(L)$ and $R(L)$, respectively.

TO DO !!!
Plotting the real gain of the predicted top-k ranking and real gain of the absolute ranking of the top k...

DCG for each L, and plotting it to find the optimal L (maximizing), where the relevance in the formula of DCG would be for us the distance between the real gain of the predicted and the real absolute rankings!!! (check the formula in the Recommender Systems 2012 Linyuan Lu paper)

For a recommendation list of length $L$, $DCG$~\cite{Moffat2008ACMJournal} is defined as

\begin{equation*}
    DCG(b,L) = \sum^{b}_{n=1}{r_n} + \sum^{L}_{n=b+1}{\frac{r_n}{log_{b}n}},
\end{equation*}

where $r_n$ indicates the relevance of the $n$-th ranked object ($r_n=1$ for a relevant object and zero otherwise) and $b$ is a persistence parameter which was suggested to be $2$. The intention of $DCG$ is that highly ranked relevant objects give more satisfaction and utility than badly ranked ones.
}
